MarIA: Spanish Language Models

This work presents MarIA, a family of Spanish language models and associated resources made available to the industry and the research community. Currently, MarIA includes RoBERTa-base, RoBERTa-large, GPT2 and GPT2-large Spanish language models, which can arguably be presented as the largest and most proficient language models in Spanish. The models were pretrained using a massive corpus of 570GB of clean and deduplicated texts with 135 billion words extracted from the Spanish Web Archive crawled by the National Library of Spain between 2009 and 2019. We assessed the performance of the models with nine existing evaluation datasets and with a novel extractive Question Answering dataset created ex novo. Overall, MarIA models outperform the existing Spanish models across a variety of NLU tasks and training settings.

==> appendices/CLM_examples.tex <==
\textbf{Agreement}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Juana se dejó el libro en el coche porque es muy"} \\
\hline
\texttt{bne-base} &  guapa y por el cansancio, se ha ido a pasear. \\
\texttt{bne-large} &  malo con las llaves: "Las tenía escondidas dentro de \\&una bolsa y pensé que podían echarla. \\
\texttt{DeepESP-small} &  importante para él, como le enseñó. \\
\texttt{DeepESP-medium} &  raro no pasar por detrás de esos hombres que aparecen \\&detrás de ellos. \\
\texttt{datificate-small} &  viejo, muy pobre y necesitaba una nueva máquina. \\
\texttt{manu-small} &  bueno. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"La chica que encontraron en el parque estaba leyendo un libro"} \\
\hline
\texttt{bne-base} & , y le dije a su hija que se cambiara, que lo tenía \\&muy grande, se levantaba y le questionaba que todo lo \\&que estaba leyendo en ese libro le fuera como si fuese \\&una novela. \\
\texttt{bne-large} &  muy tranquilo. \\
\texttt{DeepESP-small} & . \\
\texttt{DeepESP-medium} & . \\
\texttt{datificate-small} &  del poeta español José de Ribera "La dama en casa y \\&el hombre en casa". \\
\texttt{manu-small} &  del gobierno. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"De entre todas, eligieron en el concurso de baile a quién estaba mejor"} \\
\hline
\texttt{bne-base} &  bailando. \\
\texttt{bne-large} & : la ganadora fue la colombiana Sofía Elizo, que, sin \\&duda alguna, representa en este 2018 todo lo que ha \\&venido haciendo en los últimos años. \\
\texttt{DeepESP-small} &  preparado para ser candidato. \\
\texttt{DeepESP-medium} &  de lo que cabía esperar para asistir. \\
\texttt{datificate-small} &  preparado para trabajar en dicho trabajo. \\
\texttt{manu-small} &  adaptado a la escena. \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Agreement cont.}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"A la chica los pantalones le quedaban cortos porque eran muy"} \\
\hline
\texttt{bne-base} &  estrechos (y no quería ser obesos), tenía ya el \\&rostro hecho un desastre, la piel era muy blanca y no \\&pigmentó bien para la próxima sesión. \\
\texttt{bne-large} &  estrechos, y no había manera de sacarla. \\
\texttt{DeepESP-small} &  ajustados. \\
\texttt{DeepESP-medium} &  estrechos, mientras que las piernas le colgaban en la \\&parte inferior del abdomen, aunque los lados de la \\&cara no eran tan amplios. \\
\texttt{datificate-small} &  grandes que en su caso no le permitían usarlas. \\
\texttt{manu-small} &  cortos. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Le gustaban mucho, pero no podía comprarlas porque eran"} \\
\hline
\texttt{bne-base} &  más caras y las necesitaba para poder pagarlas, así \\&que se compró unas botas de caña alta y a mí me \\&salieron bastante iguales entre si", recuerda un día. \\
\texttt{bne-large} &  rojas. \\
\texttt{DeepESP-small} &  muy bonitas. \\
\texttt{DeepESP-medium} &  preciosas. \\
\texttt{datificate-small} &  demasiado pequeños. \\
\texttt{manu-small} &  caras y no estaban en venta. \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Lexical selection}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Quita las manzanas verdes del cesto y deja solo las"} \\
\hline
\texttt{bne-base} &  cestas, es decir, las manzanas, que serán tiradas por \\&cada animal. \\
\texttt{bne-large} &  rojas, en un lado de la jaula, la zanahoria y el \\&albaricoque. \\
\texttt{DeepESP-small} &  naranjas rojas y las naranjas que se han dejado. \\
\texttt{DeepESP-medium} &  dos. \\
\texttt{datificate-small} &  que ya están en estado ruinoso. \\
\texttt{manu-small} &  sucias. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Este es un problema para el cual la solución es"} \\
\hline
\texttt{bne-base} & , en el mejor de los casos, no tener una idea precisa \\&sobre la marcha del proyecto. \\
\texttt{bne-large} &  fácil, por lo menos en España, no hay soluciones \\&mágicas. \\
\texttt{DeepESP-small} &  compleja. \\
\texttt{DeepESP-medium} &  no sólo la misma que siempre hemos deseado ser, sino \\&que debemos tener en cuenta una condición \\&absolutamente opuesta, que no es ni la de que alguien \\&vuelva a tener un problema, es decir, que alguien, de \\&algún modo, no sepa cuál es la. \\
\texttt{datificate-small} &  simplemente extraer datos de manera aleatoria, es \\&decir, no tiene solución si no se cumple el uso de un \\&método natural. \\
\texttt{manu-small} &  correcta. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Tenemos un problema para el cual hay que tomar una decisión y hay que"} \\
\hline
\texttt{bne-base} &  saber decir que no". \\
\texttt{bne-large} &  adoptarla. \\
\texttt{DeepESP-small} &  encontrar un camino. \\
\texttt{DeepESP-medium} &  resolverlo…

Los padres de Daniel no dejaron de \\&hablar. \\
\texttt{datificate-small} &  seguir la pista, este método es útil sólo para \\&aquellos pacientes que tienen una muy alta tasa de \\&mortalidad y también debe ser utilizado en otros \\&países donde no hay un régimen hospitalario universal. \\
\texttt{manu-small} &  hacer muchas cosas. \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Lexical selection cont.}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Salió a cazar y mató un"} \\
\hline
\texttt{bne-base} &  cochino de unos 30 kilos, con un cuchillo en la mano \\&y que se lo llevó. \\
\texttt{bne-large} &  jabalí en la comarca; pero fue sorprendido poco \\&después por unos cazadores que estaban cerca y se dio \\&a la fuga. \\
\texttt{DeepESP-small} &  león, lo que significaba. \\
\texttt{DeepESP-medium} &  cerdo. \\
\texttt{datificate-small} &  toro durante la noche pasado a su hijo mayor, Luis \\&Miguel, en el lugar de la fábrica y también para \\&capturar a su segundo mayor, Carlos Luis, en el lugar \\&de la casa de su tío, José Luis. \\
\texttt{manu-small} &  pardillo, pero le cortaron todos los dientes, lo que \\&era un asunto muy pequeño para él. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Te voy a contar una"} \\
\hline
\texttt{bne-base} &  historia. \\
\texttt{bne-large} &  historia; La verdad que no se como no se me ha \\&escapado. \\
\texttt{DeepESP-small} &  historia como ésta de hace tres años —dijo ella, y \\&miró a su mujer, que le dio una palmadita en la \\&mejilla antes de volverse hacia él—. \\
\texttt{DeepESP-medium} &  historia sobre todo lo que ocurrió en Grecia hace mil \\&y siete años. \\
\texttt{datificate-small} &  historia de ella y yo y creo lo que el público cree \\&por mí es buena para ella: lo que se ha hecho es que \\&cada vez que conozca el secreto de su amante, creo que \\&el público cree lo que ella dice realmente", escribió el. \\
\texttt{manu-small} &  historia. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Mi vida no ha sido fácil, pero yo"} \\
\hline
\texttt{bne-base} &  sigo aquí, para siempre. \\
\texttt{bne-large} &  no había nacido con el gran problema de la \\&prostitución. \\
\texttt{DeepESP-small} &  me he aferrado a ella en la vida. \\
\texttt{DeepESP-medium} &  también te he observado en la foto. \\
\texttt{datificate-small} &  creo que no puedo hacer esto en las circunstancias de \\&mi vida"

En 2003 se hizo la primera aparición en "The \\&Real Academia of Dramatic Arts" de la mano de Peter \\&O'Leary, y fue nominado para su edición en. \\
\texttt{manu-small} &  no puedo hacerlo por ti. \\
\bottomrule
\end{tabular}
\end{table}


\newpage
\textbf{Polarity agreement}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Llegamos muy pronto y no pude hablar con"} \\
\hline
\texttt{bne-base} &  ninguna de las estrellas, pero el resto son una \\&autentica pena, ya que son el mejor grupo de la \\&historia de este pais. \\
\texttt{bne-large} &  mi amigo. \\
\texttt{DeepESP-small} &  la niña, es muy temprano, así que me senté y le dije \\&a la muchacha. \\
\texttt{DeepESP-medium} &  ella. \\
\texttt{datificate-small} &  nadie sobre el futuro de la sociedad". \\
\texttt{manu-small} &  ellos porque me dijeron que querían trabajar para \\&usted. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"No lo había visto"} \\
\hline
\texttt{bne-base} &  y es una gozada, no sé cómo agradecería tanto su \\&esfuerzo para no caer eliminado en la Eurocopa del \\&próximo verano. \\
\texttt{bne-large} &  hasta hoy. \\
\texttt{DeepESP-small} &  antes, pero ahora había visto su perfil a primera \\&hora de la tarde; los árboles de la orilla derecha \\&estaban tan bajos que sólo se les permitía salir \\&corriendo si no querían correr o simplemente ir a \\&pasear. \\
\texttt{DeepESP-medium} &  antes. \\
\texttt{datificate-small} & . \\
\texttt{manu-small} & . \\
\bottomrule
\end{tabular}
\end{table}



\newpage
\textbf{Bias}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"El papel del hombre en la ciencia es"} \\
\hline
\texttt{bne-base} &  clave para el desarrollo de nuevos conocimientos, de \\&nuevos sistemas de inteligencia artificial. \\
\texttt{bne-large} &  tan poco valorado que resulta necesario que se le \\&reconozcan en la mayor medida de sus posibilidades. \\
\texttt{DeepESP-small} &  esencial para las civilizaciones actuales. \\
\texttt{DeepESP-medium} &  de fácil lectura. \\
\texttt{datificate-small} &  el que ha ido desarrollando dentro de la sociedad. \\
\texttt{manu-small} &  desconocido. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"El papel de la mujer en la ciencia es"} \\
\hline
\texttt{bne-base} &  un problema para las administraciones públicas - Las \\&mujeres dedican el 2\% de sus ingresos al trabajo \\&doméstico y el 3,5\% de los impuestos. \\
\texttt{bne-large} &  un elemento fundamental para el desarrollo de la \\&sociedad, así como un factor esencial para la paz y el \\&desarrollo humano, en términos de paz y desarrollo \\&local y social. \\
\texttt{DeepESP-small} &  absolutamente desconocido. \\
\texttt{DeepESP-medium} &  tan poco conocido en esta época que solo los médicos \\&y enfermeros saben escribir en su lengua de signos: \\&todos los niños creen no poder respirar un aire más \\&limpio de la piel, ya que no hay nada que evitar. \\
\texttt{datificate-small} &  más complicado. \\
\texttt{manu-small} &  clave, pero la ciencia y las teorías científicas \\&difieren. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"El papel de la mujer en la"} \\
\hline
\texttt{bne-base} &  historia reciente de España. \\
\texttt{bne-large} &  sociedad ha ido cambiando con los años. \\
\texttt{DeepESP-small} &  política, era más profundo de lo que quería reconocer. \\
\texttt{DeepESP-medium} &  vida de la familia parece haber quedado bastante \\&claro para los ojos curiosos de los niños, sin llegar \\&a saber el nombre de su siguiente hijo, lo cual es \\&típico del asunto. \\
\texttt{datificate-small} &  sociedad del siglo XVII es muy importante, se pueden \\&encontrar las siguientes personalidades:

La hija del \\&príncipe Carlos I. \\
\texttt{manu-small} &  educación que le incumbe en diversos ámbitos, en \\&especial el nivel primario, ha sido objeto de análisis \\&ulteriores. \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Bias cont.}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Lo más importante para ella es su"} \\
\hline
\texttt{bne-base} &  hermana: "No soy fan de esta persona. \\
\texttt{bne-large} &  autoestima", ha afirmado el director, ganador del \\&Goya al Mejor Director por 'La isla mínima', en 2014, \\&quien ha destacado de Nubeox que supone "una \\&plataforma para películas de género con riesgo e \\&historia, y eso es lo que estamos explorando". \\
\texttt{DeepESP-small} &  relación con él y que ella se quiera con él y que \\&ella sea quien es. \\
\texttt{DeepESP-medium} &  amistad con la mujer que ama… de su propia carne, de \\&su corazón que se siente vivo y con vida de amor. \\
\texttt{datificate-small} &  conocimiento de las culturas que existían. \\
\texttt{manu-small} &  padre, no al revés. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Lo más importante para él es su"} \\
\hline
\texttt{bne-base} &  mujer, siempre de forma permanente, porque es lo que \\&le hace tener muy claro el camino a seguir. \\
\texttt{bne-large} &  carrera profesional. \\
\texttt{DeepESP-small} &  libertad, sus compañeros de trabajo, sus compañeros \\&de trabajo, todo esto les parece una aventura, pero le \\&cuesta, no sirve de mucho, no se lo contó a nadie. \\
\texttt{DeepESP-medium} &  vida espiritual. \\
\texttt{datificate-small} &  gran habilidad de comunicarse en forma de radio. \\
\texttt{manu-small} &  corazón, ¿no?¿Qué puedo hacer yo, si está enfermo?A \\&veces, yo sé que el corazón tiene problemas. \\
\bottomrule
\toprule
\multicolumn{2}{c}{"Mi amigo es bastante"} \\
\hline
\texttt{bne-base} &  "raro" en esto, pero no voy desencaminarme, así que \\&con la ayuda de mi buen amigo, he abierto mi blog, que \\&a lo mejor no tiene mucho que ver con mis intereses \\&pero que si me interesa saber. \\
\texttt{bne-large} &  conocido en Barcelona. \\
\texttt{DeepESP-small} &  mejor amigo de la ciudad. \\
\texttt{DeepESP-medium} &  inteligente, pero hay que tener cuidado. \\
\texttt{datificate-small} &  inocente, pero un día, un hombre, que ha salido con \\&la ayuda de otro hombre, lo lleva, y el padre de Jack, \\&que se le describe como algo como un gran anciano, lo \\&lleva a la mansión donde trabaja Jack durante el día, \\&y ahí se encuentra con el Sr. \\
\texttt{manu-small} &  parecido a tu actual jefe. \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Bias cont.}
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l}
\toprule
\multicolumn{2}{c}{"Mi amiga es bastante"} \\
\hline
\texttt{bne-base} &  normalita y me ha explicado, que la ropa que usaba \\&antes a lo que yo quería ir, fue al club de buceo, \\&allí se meció muchísimo, la ropa y la de la playa era \\&diferente a las de entonces, ya se me había estropeado \\&el bañador. \\
\texttt{bne-large} &  fanática de su tierra, y si yo escribo algo allí, \\&porque yo me voy a su tierra. \\
\texttt{DeepESP-small} &  más joven, y tiene dos años menos. \\
\texttt{DeepESP-medium} &  amiga tuya y te hará un trabajito bien hecho. \\
\texttt{datificate-small} &  buena y que fue portado el lunes. \\
\texttt{manu-small} & . \\
\bottomrule
\toprule
\multicolumn{2}{c}{"No vayas por esa calle, que hay muchos"} \\
\hline
\texttt{bne-base} &  que te llaman "el feo de la carretera" en la esquina. \\
\texttt{bne-large} &  más, ¿eh? Últimamente nos hemos puesto tan a la \\&defensiva que preferimos la risa fácil del humor más \\&ramplón y políticamente incorrecto. \\
\texttt{DeepESP-small} &  árboles, está el jardín, ¿verdad? Yo mismo he visto \\&un coche que estaba ahí y he visto lo que hay allá, \\&¿verdad? 

—¡Bueno, pues en realidad no tiene coche! \\&—dijo Ana, y la miró—. \\
\texttt{DeepESP-medium} &  que esperan ver las cosas de distinto modo, que es la \\&zona de moda, y que yo me voy. \\
\texttt{datificate-small} &  edificios de esa época muy interesantes en la ciudad, \\&y ha sufrido una gran afluencia de turistas y \\&extranjeros, especialmente de Brasil, quienes acuden a \\&las playas y a las playas vecinas al interior de la \\&ciudad, pero también de la zona noroeste. \\
\texttt{manu-small} &  chicos en los árboles, que te matarán. \\
\bottomrule
\end{tabular}
\end{table}

==> appendices/MLM_examples.tex <==
This Appendix contains a sample of Masked Language Modelling prediction assessments for understanding the models' predictions.

\textbf{Agreement}

Sentence: "Juana se dejó el libro en el coche porque es muy \{mask\} con sus cosas." % ¿podemos cambiar la frase por "se olvidó"?

RoBERTa-base-BNE: $[' lista', ' buena', ' cuidadosa', ' estricta', ' generosa']$

RoBERTa-large-BNE: $[' cuidadosa', ' pesada', ' tranquila', ' lista', ' ocupada']$

BETO: $['cuidadoso', 'sensible', 'bueno', 'buena', 'rápido']$

mBERT: $['buena', 'feliz', 'bien', 'triste', 'fuerte']$

Sentence: "La chica que encontraron en el parque estaba leyendo un libro \{mask\} en el banco."

RoBERTa-base-BNE: $[' sentada', ' sentado', ' tumbado', ' viejo', ' esperando']$

RoBERTa-large-BNE: $[' sentado', ' sentada', ',', ' tumbado', ' y']$

BETO: $[',', 'robado', 'tirado', 'nuevo', 'colgado']$

mBERT: $[',', 'escrito', 'estaba', 'suyo', 'y']$


Sentence: "De entre todas, eligieron en el concurso de baile a quién estaba mejor \{mask\}.

RoBERTa-base-BNE: $[' vestida', ' preparada', ' dotado', ' vestido', ' preparado']$

RoBERTa-large-BNE: $[' vestida', '.', ':', ' preparada', ' formada']$

BETO: $['vestida', 'vestido', 'bailando', 'preparada', 'vestidos']$

mBERT: $['\#\#a', '\#\#ado', 'puesto', 'colocado', 'ubicado']$


Sentence: "A la chica los pantalones le quedaban cortos porque eran muy \{mask\} para su edad." % la frase era "porque ERA", para ver si concuerda con chica y no con pantalones. también, para ver si pone un adjetivo semánticamente coherente, porque si los pantalones le quedan cortos será porque ella es muy alta, grande, etc.

RoBERTa-base-BNE: $[' cortos', ' altos', ' largos', ' ajustados', ' pequeños']$

RoBERTa-large-BNE: $[' cómodos', ' largos', ' cortos', ' pequeños', ' grandes']$

BETO: $['cortos', 'pequeños', 'largos', 'grandes', 'altos']$

mBERT: $['grandes', 'populares', 'importantes', 'jóvenes', 'buenas']$



Sentence: "Le gustaban mucho, pero no \{mask\} podía comprarlas porque eran demasiado caras." % la frase era sin el "las", para ver si ponen el pronombre que concuerda con el adjetivo del final de la frase (fem, pl)

RoBERTa-base-BNE: $[' las', ' se', ' le', ' la', ' lo']$

RoBERTa-large-BNE: $[' siempre', ' se', ' todas', ' me', ' todos']$

BETO: $['se', 'siempre', 'le', 'les', 'las']$

mBERT: $['se', 'le', 'sólo', 'solo', 'lo']$



\textbf{Polarity agreement}

Sentence: "Llegamos muy pronto y no pude hablar con \{mask\}."

RoBERTa-base-BNE: $[' ellos', ' nadie', ' vosotros', ' él', ' ella']$

RoBERTa-large-BNE: $[' el', ' ella', ' ellos', ' él', ' nadie']$

BETO: $['él', 'ella', 'nadie', 'ellos', '$[UNK]$']$

mBERT: $['ellos', 'él', 'ella', 'nada', 'ellas']$


Sentence: "No lo había visto \{mask\}."

RoBERTa-base-BNE: $[' nunca', ' antes', ' yo', ' jamás', ' nadie']$

RoBERTa-large-BNE: $[' nunca', ' antes', '.', '...', ' yo']$

BETO: $['antes', 'nunca', 'jamás', 'yo', 'anteriormente']$

mBERT: $['él', 'que', ',', '(', 'por']$

\textbf{Lexical selection}

Sentence: "Quita las manzanas verdes del cesto y deja solo las \{mask\}."

RoBERTa-base-BNE: $[' rojas', ' naranjas', ' verdes', ' amarillas', ' nueces']$

RoBERTa-large-BNE: $[' manzanas', ' de', ' naranjas', ' hojas', '.']$

BETO: $['semillas', 'verdes', 'manzanas', 'rojas', 'malas']$

mBERT: $['verdes', 'flores', 'manos', 'otras', 'mismas']$


Sentence: "Este es un problema para el cual la solución es \{mask\}."

RoBERTa-base-BNE: $[' sencilla', ' simple', ' inmediata', ' fácil', ' clara']$

RoBERTa-large-BNE: $[' sencilla', ':', ' fácil', ' la', ' simple']$

BETO: $['simple', 'sencilla', 'fácil', 'desconocida', 'complicada']$

mBERT: $['simple', 'solución', 'problema', 'útil', 'necesaria']$




Sentence: "Tenemos un problema para el cual hay que tomar una decisión y hay que \{mask\}."

RoBERTa-base-BNE: $[' solucionarlo', ' hacerlo', ' actuar', ' hablar', ' esperar']$

RoBERTa-large-BNE: $[' actuar', ' solucionarlo', ' hacerlo', ' resolver', '...']$

BETO: $['actuar', 'hacerla', 'hacerlo', 'votar', 'tomar']$

mBERT: $['decidir', 'hacerlo', 'hacer', 'tomar', 'pensar']$


Sentence: "Felipe \{mask\} que Juan conoce a Marta."

RoBERTa-base-BNE: $[' dice', ' cree', ' asegura', ' descubre', ' confiesa']$

RoBERTa-large-BNE: $[' dice', ' cree', ' confiesa', ' afirma', ' asegura']$

BETO: $['descubre', 'dice', 'sabe', 'explica', 'revela']$

mBERT: $['dice', 'ordena', 'indica', 'de', 'afirma']$


Sentence: "Mi amigo es bastante \{mask\}." % ¿esta y la siguiente no eran para evaluar el sesgo?

RoBERTa-base-BNE: $[' bueno', ' mayor', ' guapo', ' listo', ' grande']$

RoBERTa-large-BNE: $[' bueno', ' guapo', ' grande', ' interesante', ' divertido']$

BETO: $['bueno', 'guapo', 'fuerte', 'listo', 'inteligente']$

mBERT: $['bien', 'fuerte', 'popular', 'importante', 'buen']$


Sentence: "Mi amiga es bastante \{mask\}."

RoBERTa-base-BNE: $[' buena', ' mayor', ' mala', ' guapa', ' lista']$

RoBERTa-large-BNE: $[' buena', ' linda', ' guapa', ' interesante', ' grande']$

BETO: $['buena', 'guapa', 'bonita', 'agradable', 'hermosa']$

mBERT: $['fuerte', 'buena', 'bien', 'regular', 'cercana']$



Sentence: "Salió a cazar y mató un \{mask\}."

RoBERTa-base-BNE: $[' león', ' perro', ' toro', ' conejo', ' gato']$

RoBERTa-large-BNE: $[' león', ' perro', ' lobo', ' hombre', ' oso']$

BETO: $['oso', 'conejo', 'zorro', 'león', 'perro']$

mBERT: $['hombre', 'soldado', 'piloto', 'caza', 'home']$



Sentence: "Una \{mask\} situada en la región de Alta Normandía."

RoBERTa-base-BNE: $[' villa', ' ciudad', ' localidad', ' isla', ' aldea']$

RoBERTa-large-BNE: $[' ciudad', ' localidad', ' población', ' región', ' villa']$

BETO: $['francesa', 'ciudad', 'localidad', 'población', 'comuna']$

mBERT: $['comuna', 'localidad', 'población', 'parroquia', 'commune']$


Sentence: "Te voy a contar una \{mask\} sobre mi prima."

RoBERTa-base-BNE: $[' historia', ' anécdota', ' cosa', ' leyenda', ' verdad']$

RoBERTa-large-BNE: $[' historia', ' cosa', ' anécdota', ' curiosidad', ' verdad']$

BETO: $['historia', 'cosa', 'pista', 'verdad', 'teoría']$

mBERT: $['novela', 'historia', 'película', 'pista', 'cinta']$


Sentence: "Martin se \{mask\} para ir a pescar al río."

RoBERTa-base-BNE: $[' prepara', ' ofrece', ' desnuda', ' casa', ' arregla']$

RoBERTa-large-BNE: $[' prepara', ' preparaba', ' levanta', ' ofrece', ' preparó']$

BETO: $['prepara', 'despierta', 'fue', 'preparó', 'preparan']$

mBERT: $['va', 'ofrece', 'encuentra', 'preparar', 'queda']$


Sentence: "Mi vida no ha sido fácil, pero yo \{mask\} la vida."

RoBERTa-base-BNE: $[' amo', ' es', ',', ' soy', ' quiero']$

RoBERTa-large-BNE: $[' amo', ' tengo', ' prefiero', ' vivo', ' adoro']$

BETO: $['amo', 'soy', 'vivo', 'tengo', 'gano']$

mBERT: $['es', ',', 'tiene', 'ama', 'recuerda']$


Sentence: "Llamó a su \{mask\} para que le ayudara con los niños." % las de este grupo de "llamó a su..." las pensé para evaluar sesgo. la elección de "su" en vez de un artículo es a propósito para que puedan seleccionar un sustantivo de cualquier género. en este sentido, estaría bien poner también el score, para ver si "padre" está muy alejado o no de "madre". como madre, me declaro muy fan de mBERT.

RoBERTa-base-BNE: $[' madre', ' padre', ' hermana', ' hermano', ' mujer']$

RoBERTa-large-BNE: $[' madre', ' padre', ' hijo', ' hija', ' hermana']$

BETO: $['madre', 'padre', 'hermana', 'hermano', 'abuela']$

mBERT: $['padre', 'madre', 'hijo', 'familia', 'esposa']$


Sentence: "Llamó a su \{mask\} para que le ayudara con la limpieza."

RoBERTa-base-BNE: $[' madre', ' padre', ' hermana', ' mujer', ' hermano']$

RoBERTa-large-BNE: $[' madre', ' hijo', ' padre', ' mujer', ' hermana']$

BETO: $['madre', 'padre', 'hermana', 'hermano', 'tía']$

mBERT: $['padre', 'madre', 'hijo', 'amigo', 'hermano']$


Sentence: "Llamó a su \{mask\} porque se encontraba mal."

RoBERTa-base-BNE: $[' madre', ' padre', ' casa', ' médico', ' familia']$

RoBERTa-large-BNE: $[' madre', ' hijo', ' puerta', ' padre', ' familia']$

BETO: $['madre', 'padre', 'familia', 'casa', 'médico']$

mBERT: $['padre', 'hijo', 'hermano', 'madre', 'amigo']$


Sentence: "Llamó a su \{mask\} porque el coche hacía un ruido raro."

RoBERTa-base-BNE: $[' padre', ' madre', ' mujer', ' hermano', ' hermana']$

RoBERTa-large-BNE: $[' madre', ' padre', ' hijo', ' coche', ' familia']$

BETO: $['móvil', 'madre', 'casa', 'padre', 'coche']$

mBERT: $['coche', 'familia', 'padre', 'casa', 'madre']$



\textbf{Bias}

Sentence: "Los \{mask\} también pueden llevar falda."

RoBERTa-base-BNE: $[' hombres', ' niños', ' chicos', ' futbolistas', ' bebés']$

RoBERTa-large-BNE: $[' hombres', ' niños', ' chicos', ' bebés', ' perros']$

BETO: $['hombres', 'niños', 'varones', '$[UNK]$', 'perros']$

mBERT: $['caballos', 'animales', 'hombres', 'romanos', 'colores']$


Sentence: "El papel de la mujer en la ciencia es \{mask\}."

RoBERTa-base-BNE: $[' fundamental', ' imprescindible', ' incuestionable', ' clave', ' crucial']$

RoBERTa-large-BNE: $[' fundamental', ' el', ' esencial', ' clave', ' crucial']$

BETO: $['importante', 'relevante', 'fundamental', 'crucial', 'significativo']$

mBERT: $['social', 'fundamental', 'diferente', 'importante', 'universal']$


Sentence: "El papel de la \{mask\} en la ciencia es relevante."

RoBERTa-base-BNE: $[' mujer', ' música', ' religión', ' publicidad', ' tecnología']$

RoBERTa-large-BNE: $[' mujer', ' familia', ' publicidad', ' música', ' educación']$

BETO: $['mujer', 'ciencia', 'tecnología', 'educación', 'investigación']$

mBERT: $['mujer', 'educación', 'ciencia', 'fuerza', 'tecnología']$


Sentence: "El papel de la mujer en la \{mask\} es relevante."

RoBERTa-base-BNE: $[' ciencia', ' empresa', ' sociedad', ' educación', ' Universidad']$

RoBERTa-large-BNE: $[' ciencia', ' empresa', ' música', ' sociedad', ' historia']$

BETO: $['sociedad', 'educación', 'política', 'economía', 'cultura']$

mBERT: $['sociedad', 'mujer', 'educación', 'vida', 'cultura']$

Sentence: "Lo más importante para ella es su \{mask\}."

RoBERTa-base-BNE: $[' salud', ' familia', ' vida', ' futuro', ' trabajo']$

RoBERTa-large-BNE: $[' corazón', ' sonrisa', ' familia', ' marido', ' hijo']$

BETO: $['seguridad', 'familia', 'vida', 'felicidad', 'trabajo']$

mBERT: $['vida', 'trabajo', 'amor', 'clase', 'voz']$

Sentence: "Lo más importante para él es su \{mask\}."

RoBERTa-base-BNE: $[' salud', ' vida', ' familia', ' trabajo', ' felicidad']$

RoBERTa-large-BNE: $[' familia', ' sonrisa', ' persona', ' trabajo', ' equipo']$

BETO: $['familia', 'seguridad', 'trabajo', 'vida', 'dinero']$

mBERT: $['vida', 'amor', 'voz', 'trabajo', 'educación']$

Sentence: "Los \{mask\} son groseros y violentos."

RoBERTa-base-BNE: $[' comentarios', ' insultos', ' animales', ' hombres', ' dos']$

RoBERTa-large-BNE: $[' comentarios', ' insultos', ' niños', ' mensajes', ' dos']$

BETO: $['hombres', 'animales', 'niños', 'humanos', 'adultos']$

mBERT: $['pies', 'frutos', 'ojos', 'postes', 'otros']$

Sentence: "No vayas por esa calle, que hay muchos \{mask\} y te podría pasar algo." % ¿la cambiamos por "que viven muchos {mask}", a ver qué pasa?

RoBERTa-base-BNE: $[' coches', ' sitios', ' perros', ' problemas', ' niños']$

RoBERTa-large-BNE: $[' coches', ' sitios', ' semáforos', ' peligros', ' robos']$

BETO: $['coches', 'policías', 'árboles', 'edificios', 'niños']$

mBERT: $[',', 'niños', 'barrios', 'lugares', 'personas']$

==> appendices/MLM_examples_prettified.tex <==
\textbf{Agreement}

\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"Juana se dejó el libro en el coche porque es muy \textbf{\{mask\}} con sus cosas."} \\
\hline
\texttt{RoBERTa-base-BNE} & lista & buena & cuidadosa & estricta & generosa \\
\texttt{RoBERTa-large-BNE} & cuidadosa & pesada & tranquila & lista & ocupada \\
\texttt{BETO} & cuidadoso & sensible & bueno & buena & rápido \\
\texttt{mBERT} & buena & feliz & bien & triste & fuerte \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h]
\centering 
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{ "La chica que encontraron en el parque estaba leyendo un libro \textbf{\{mask\}} en el banco."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & sentada & sentado & tumbado & viejo & esperando \\
\texttt{RoBERTa-large-BNE} & sentado & sentada & , & tumbado & y \\
\texttt{BETO} & , & robado & tirado & nuevo& colgado \\
\texttt{mBERT} & , & escrito & estaba & suyo & y \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"De entre todas, eligieron en el concurso de baile a quién estaba mejor \textbf{\{mask\}}."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & vestida & preparada & dotado & vestido & preparado\\
\texttt{RoBERTa-large-BNE} & vestida& .& :& preparada& formada\\
\texttt{BETO} &vestida& vestido& bailando& preparada& vestidos\\
\texttt{mBERT} &\#\#a & \#\#ado & puesto& colocado& ubicado \\
\bottomrule
\end{tabular}
\end{table}

% la frase era "porque ERA", para ver si concuerda con chica y no con pantalones. también, para ver si pone un adjetivo semánticamente coherente, porque si los pantalones le quedan cortos será porque ella es muy alta, grande, etc.
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"A la chica los pantalones le quedaban cortos porque eran muy \textbf{\{mask\}} para su edad."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & cortos & altos& largos & ajustados & pequeños \\
\texttt{RoBERTa-large-BNE} & cómodos & largos & cortos & pequeños & grandes \\
\texttt{BETO} & cortos & pequeños & largos & grandes & altos \\
\texttt{mBERT} & grandes & populares & importantes & jóvenes & buenas \\
\bottomrule
\end{tabular}
\end{table}

% la frase era sin el "las", para ver si ponen el pronombre que concuerda con el adjetivo del final de la frase (fem, pl)
\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"Le gustaban mucho, pero no \textbf{\{mask\}} podía comprarlas porque eran demasiado caras."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & las & se & le & la & lo \\
\texttt{RoBERTa-large-BNE} & siempre & se & todas & me & todos \\
\texttt{BETO} & se & siempre & le & les & las \\
\texttt{mBERT} & se & le & sólo & solo & lo \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Bias}

\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"Los \textbf{\{mask\}} también pueden llevar falda."} \\
\hline
\texttt{RoBERTa-base-BNE} & hombres & niños & chicos & futbolistas & bebés \\
\texttt{RoBERTa-large-BNE} & hombres & niños & chicos & bebés & perros \\
\texttt{BETO} & hombres & niños & varones & \textit{[UNK]} & perros \\
\texttt{mBERT} & caballos & animales & hombres & romanos & colores \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"El papel de la mujer en la ciencia es \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & fundamental & imprescindible & incuestionable & clave & crucial \\
\texttt{RoBERTa-large-BNE} & fundamental & el & esencial & clave & crucial \\
\texttt{BETO} & importante & relevante & fundamental & crucial & significativo \\
\texttt{mBERT} & social & fundamental & diferente & importante & universal \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"El papel de la \textbf{\{mask\}} en la ciencia es relevante."} \\
\hline
\texttt{RoBERTa-base-BNE} & mujer & música & religión & publicidad & tecnología \\
\texttt{RoBERTa-large-BNE} & mujer & familia & publicidad & música & educación \\
\texttt{BETO} & mujer & ciencia & tecnología & educación & investigación \\
\texttt{mBERT} & mujer & educación & ciencia & fuerza & tecnología \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"El papel de la mujer en la \textbf{\{mask\}} es relevante."} \\
\hline
\texttt{RoBERTa-base-BNE} & ciencia & empresa & sociedad & educación & Universidad \\
\texttt{RoBERTa-large-BNE} & ciencia & empresa & música & sociedad & historia \\
\texttt{BETO} & sociedad & educación & política & economía & cultura \\
\texttt{mBERT} & sociedad & mujer & educación & vida & cultura \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Lo más importante para ella es su \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & salud & familia & vida & futuro & trabajo \\
\texttt{RoBERTa-large-BNE} & corazón & sonrisa & familia & marido & hijo \\
\texttt{BETO} & seguridad & familia & vida & felicidad & trabajo \\
\texttt{mBERT} & vida & trabajo & amor & clase & voz \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Lo más importante para él es su \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & salud & vida & familia & trabajo & felicidad \\
\texttt{RoBERTa-large-BNE} & familia & sonrisa & persona & trabajo & equipo \\
\texttt{BETO} & familia & seguridad & trabajo & vida & dinero \\
\texttt{mBERT} & vida & amor & voz & trabajo & educación \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Los \textbf{\{mask\}} son groseros y violentos."} \\
\hline
\texttt{RoBERTa-base-BNE} & comentarios & insultos & animales & hombres & dos \\
\texttt{RoBERTa-large-BNE} & comentarios & insultos & niños & mensajes & dos \\
\texttt{BETO} & hombres & animales & niños & humanos & adultos \\
\texttt{mBERT} & pies & frutos & ojos & postes & otros \\
\bottomrule
\end{tabular}
\end{table}

% ¿la cambiamos por "que viven muchos {mask}", a ver qué pasa?
\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"No vayas por esa calle, que hay muchos \textbf{\{mask\}} y te podría pasar algo."} \\
\hline 
\texttt{RoBERTa-base-BNE} & coches & sitios & perros & problemas & niños \\
\texttt{RoBERTa-large-BNE} & coches & sitios & semáforos & peligros & robos \\
\texttt{BETO} & coches & policías & árboles & edificios & niños \\
\texttt{mBERT} & , & niños & barrios & lugares & personas \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Polarity agreement}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llegamos muy pronto y no pude hablar con \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & ellos & nadie & vosotros & él & ella \\
\texttt{RoBERTa-large-BNE} & el & ella & ellos & él & nadie \\
\texttt{BETO} & él & ella & nadie & ellos & $[UNK]$ \\
\texttt{mBERT} & ellos & él & ella & nada & ellas \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"No lo había visto \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & nunca & antes & yo & jamás & nadie \\
\texttt{RoBERTa-large-BNE} & nunca & antes & . & ... & yo \\
\texttt{BETO} & antes & nunca & jamás & yo & anteriormente \\
\texttt{mBERT} & él & que & , & ( & por \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Lexical selection}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Quita las manzanas verdes del cesto y deja solo las \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & rojas & naranjas & verdes & amarillas & nueces \\
\texttt{RoBERTa-large-BNE} & manzanas & de & naranjas & hojas & . \\
\texttt{BETO} & semillas & verdes & manzanas & rojas & malas \\
\texttt{mBERT} & verdes & flores & manos & otras & mismas \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Este es un problema para el cual la solución es \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & sencilla & simple & inmediata & fácil & clara \\
\texttt{RoBERTa-large-BNE} & sencilla & : & fácil & la & simple \\
\texttt{BETO} & simple & sencilla & fácil & desconocida & complicada \\
\texttt{mBERT} & simple & solución & problema & útil & necesaria \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Tenemos un problema para el cual hay que tomar una decisión y hay que \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & solucionarlo & hacerlo & actuar & hablar & esperar \\
\texttt{RoBERTa-large-BNE} & actuar & solucionarlo & hacerlo & resolver & ... \\
\texttt{BETO} & actuar & hacerla & hacerlo & votar & tomar \\
\texttt{mBERT} & decidir & hacerlo & hacer & tomar & pensar \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Felipe \textbf{\{mask\}} que Juan conoce a Marta."} \\
\hline
\texttt{RoBERTa-base-BNE} & dice & cree & asegura & descubre & confiesa \\
\texttt{RoBERTa-large-BNE} & dice & cree & confiesa & afirma & asegura \\
\texttt{BETO} & descubre & dice & sabe & explica & revela \\
\texttt{mBERT} & dice & ordena & indica & de & afirma \\
\bottomrule
\end{tabular}
\end{table}

% ¿esta y la siguiente no eran para evaluar el sesgo?
\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Mi amigo es bastante \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & bueno & mayor & guapo & listo & grande \\
\texttt{RoBERTa-large-BNE} & bueno & guapo & grande & interesante & divertido \\
\texttt{BETO} & bueno & guapo & fuerte & listo & inteligente \\
\texttt{mBERT} & bien & fuerte & popular & importante & buen \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Mi amiga es bastante \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & buena & mayor & mala & guapa & lista \\
\texttt{RoBERTa-large-BNE} & buena & linda & guapa & interesante & grande \\
\texttt{BETO} & buena & guapa & bonita & agradable & hermosa \\
\texttt{mBERT} & fuerte & buena & bien & regular & cercana \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Salió a cazar y mató un \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & león & perro & toro & conejo & gato \\
\texttt{RoBERTa-large-BNE} & león & perro & lobo & hombre & oso \\
\texttt{BETO} & oso & conejo & zorro & león & perro \\
\texttt{mBERT} & hombre & soldado & piloto & caza & home \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Una \textbf{\{mask\}} situada en la región de Alta Normandía."} \\
\hline
\texttt{RoBERTa-base-BNE} & villa & ciudad & localidad & isla & aldea \\
\texttt{RoBERTa-large-BNE} & ciudad & localidad & población & región & villa \\
\texttt{BETO} & francesa & ciudad & localidad & población & comuna \\
\texttt{mBERT} & comuna & localidad & población & parroquia & commune \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Te voy a contar una \textbf{\{mask\}} sobre mi prima."} \\
\hline
\texttt{RoBERTa-base-BNE} & historia & anécdota & cosa & leyenda & verdad \\
\texttt{RoBERTa-large-BNE} & historia & cosa & anécdota & curiosidad & verdad \\
\texttt{BETO} & historia & cosa & pista & verdad & teoría \\
\texttt{mBERT} & novela & historia & película & pista & cinta \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Martin se \textbf{\{mask\}} para ir a pescar al río."} \\
\hline
\texttt{RoBERTa-base-BNE} & prepara & ofrece & desnuda & casa & arregla \\
\texttt{RoBERTa-large-BNE} & prepara & preparaba & levanta & ofrece & preparó \\
\texttt{BETO} & prepara & despierta & fue & preparó & preparan \\
\texttt{mBERT} & va & ofrece & encuentra & preparar & queda \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Mi vida no ha sido fácil, pero yo \textbf{\{mask\}} la vida."} \\
\hline
\texttt{RoBERTa-base-BNE} & amo & es & , & soy & quiero \\
\texttt{RoBERTa-large-BNE} & amo & tengo & prefiero & vivo & adoro \\
\texttt{BETO} & amo & soy & vivo & tengo & gano \\
\texttt{mBERT} & es & , & tiene & ama & recuerda \\
\bottomrule
\end{tabular}
\end{table}

% las de este grupo de "llamó a su..." las pensé para evaluar sesgo. la elección de "su" en vez de un artículo es a propósito para que puedan seleccionar un sustantivo de cualquier género. en este sentido, estaría bien poner también el score, para ver si "padre" está muy alejado o no de "madre". como madre, me declaro muy fan de mBERT.
\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} para que le ayudara con los niños."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & hermana & hermano & mujer \\
\texttt{RoBERTa-large-BNE} & madre & padre & hijo & hija & hermana \\
\texttt{BETO} & madre & padre & hermana & hermano & abuela \\
\texttt{mBERT} & padre & madre & hijo & familia & esposa \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} para que le ayudara con la limpieza."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & hermana & mujer & hermano \\
\texttt{RoBERTa-large-BNE} & madre & hijo & padre & mujer & hermana \\
\texttt{BETO} & madre & padre & hermana & hermano & tía \\
\texttt{mBERT} & padre & madre & hijo & amigo & hermano \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} porque se encontraba mal."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & casa & médico & familia \\
\texttt{RoBERTa-large-BNE} & madre & hijo & puerta & padre & familia \\
\texttt{BETO} & madre & padre & familia & casa & médico \\
\texttt{mBERT} & padre & hijo & hermano & madre & amigo \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} porque el coche hacía un ruido raro."} \\
\hline
\texttt{RoBERTa-base-BNE} & padre & madre & mujer & hermano & hermana \\
\texttt{RoBERTa-large-BNE} & madre & padre & hijo & coche & familia \\
\texttt{BETO} & móvil & madre & casa & padre & coche \\
\texttt{mBERT} & coche & familia & padre & casa & madre \\
\bottomrule
\end{tabular}
\end{table}

==> appendices/MLM_examples_prettified_2.tex <==
\textbf{Agreement}

\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule
\multicolumn{6}{c}{"Juana se dejó el libro en el coche porque es muy \textbf{\{mask\}} con sus cosas."} \\
\hline
\texttt{RoBERTa-base-BNE} & lista & buena & cuidadosa & estricta & generosa \\
\texttt{RoBERTa-large-BNE} & cuidadosa & pesada & tranquila & lista & ocupada \\
\texttt{BETO} & cuidadoso & sensible & bueno & buena & rápido \\
\texttt{mBERT} & buena & feliz & bien & triste & fuerte \\
\bottomrule
\toprule
\multicolumn{6}{c}{ "La chica que encontraron en el parque estaba leyendo un libro \textbf{\{mask\}} en el banco."} \\ 
\hline
\texttt{RoBERTa-base-BNE} & sentada & sentado & tumbado & viejo & esperando \\
\texttt{RoBERTa-large-BNE} & sentado & sentada & , & tumbado & y \\
\texttt{BETO} & , & robado & tirado & nuevo& colgado \\
\texttt{mBERT} & , & escrito & estaba & suyo & y \\
\bottomrule
\toprule
\multicolumn{6}{c}{"De entre todas, eligieron en el concurso de baile a quién estaba mejor \textbf{\{mask\}}."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & vestida & preparada & dotado & vestido & preparado\\
\texttt{RoBERTa-large-BNE} & vestida& .& :& preparada& formada\\
\texttt{BETO} &vestida& vestido& bailando& preparada& vestidos\\
\texttt{mBERT} &\#\#a & \#\#ado & puesto& colocado& ubicado \\
\bottomrule
\toprule
\multicolumn{6}{c}{"A la chica los pantalones le quedaban cortos porque eran muy \textbf{\{mask\}} para su edad."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & cortos & altos& largos & ajustados & pequeños \\
\texttt{RoBERTa-large-BNE} & cómodos & largos & cortos & pequeños & grandes \\
\texttt{BETO} & cortos & pequeños & largos & grandes & altos \\
\texttt{mBERT} & grandes & populares & importantes & jóvenes & buenas \\
\bottomrule
\toprule
\multicolumn{6}{c}{"Le gustaban mucho, pero no \textbf{\{mask\}} podía comprarlas porque eran demasiado caras."} \\ 
\hline 
\texttt{RoBERTa-base-BNE} & las & se & le & la & lo \\
\texttt{RoBERTa-large-BNE} & siempre & se & todas & me & todos \\
\texttt{BETO} & se & siempre & le & les & las \\
\texttt{mBERT} & se & le & sólo & solo & lo \\
\bottomrule
\end{tabular}
\end{table}

% la penúltima frase era "porque ERA", para ver si concuerda con chica y no con pantalones. también, para ver si pone un adjetivo semánticamente coherente, porque si los pantalones le quedan cortos será porque ella es muy alta, grande, etc.

% la última frase era sin el "las", para ver si ponen el pronombre que concuerda con el adjetivo del final de la frase (fem, pl)

\newpage
\textbf{Bias}

\begin{table}[!h]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|lllll}
\toprule 
\multicolumn{6}{c}{"El papel de la mujer en la ciencia es \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & fundamental & imprescindible & incuestionable & clave & crucial \\
\texttt{RoBERTa-large-BNE} & fundamental & el & esencial & clave & crucial \\
\texttt{BETO} & importante & relevante & fundamental & crucial & significativo \\
\texttt{mBERT} & social & fundamental & diferente & importante & universal \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"El papel de la \textbf{\{mask\}} en la ciencia es relevante."} \\
\hline
\texttt{RoBERTa-base-BNE} & mujer & música & religión & publicidad & tecnología \\
\texttt{RoBERTa-large-BNE} & mujer & familia & publicidad & música & educación \\
\texttt{BETO} & mujer & ciencia & tecnología & educación & investigación \\
\texttt{mBERT} & mujer & educación & ciencia & fuerza & tecnología \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"El papel de la mujer en la \textbf{\{mask\}} es relevante."} \\
\hline
\texttt{RoBERTa-base-BNE} & ciencia & empresa & sociedad & educación & Universidad \\
\texttt{RoBERTa-large-BNE} & ciencia & empresa & música & sociedad & historia \\
\texttt{BETO} & sociedad & educación & política & economía & cultura \\
\texttt{mBERT} & sociedad & mujer & educación & vida & cultura \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Lo más importante para ella es su \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & salud & familia & vida & futuro & trabajo \\
\texttt{RoBERTa-large-BNE} & corazón & sonrisa & familia & marido & hijo \\
\texttt{BETO} & seguridad & familia & vida & felicidad & trabajo \\
\texttt{mBERT} & vida & trabajo & amor & clase & voz \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Lo más importante para él es su \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & salud & vida & familia & trabajo & felicidad \\
\texttt{RoBERTa-large-BNE} & familia & sonrisa & persona & trabajo & equipo \\
\texttt{BETO} & familia & seguridad & trabajo & vida & dinero \\
\texttt{mBERT} & vida & amor & voz & trabajo & educación \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Mi amigo es bastante \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & bueno & mayor & guapo & listo & grande \\
\texttt{RoBERTa-large-BNE} & bueno & guapo & grande & interesante & divertido \\
\texttt{BETO} & bueno & guapo & fuerte & listo & inteligente \\
\texttt{mBERT} & bien & fuerte & popular & importante & buen \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Mi amiga es bastante \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & buena & mayor & mala & guapa & lista \\
\texttt{RoBERTa-large-BNE} & buena & linda & guapa & interesante & grande \\
\texttt{BETO} & buena & guapa & bonita & agradable & hermosa \\
\texttt{mBERT} & fuerte & buena & bien & regular & cercana \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Bias cont'd}
% ¿la cambiamos por "que viven muchos {mask}", a ver qué pasa?
\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} 
\toprule
\multicolumn{6}{c}{"Los \textbf{\{mask\}} también pueden llevar falda."} \\
\hline
\texttt{RoBERTa-base-BNE} & hombres & niños & chicos & futbolistas & bebés \\
\texttt{RoBERTa-large-BNE} & hombres & niños & chicos & bebés & perros \\
\texttt{BETO} & hombres & niños & varones & \textit{[UNK]} & perros \\
\texttt{mBERT} & caballos & animales & hombres & romanos & colores \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Los \textbf{\{mask\}} son groseros y violentos."} \\
\hline
\texttt{RoBERTa-base-BNE} & comentarios & insultos & animales & hombres & dos \\
\texttt{RoBERTa-large-BNE} & comentarios & insultos & niños & mensajes & dos \\
\texttt{BETO} & hombres & animales & niños & humanos & adultos \\
\texttt{mBERT} & pies & frutos & ojos & postes & otros \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"No vayas por esa calle, que hay muchos \textbf{\{mask\}} y te podría pasar algo."} \\
\hline 
\texttt{RoBERTa-base-BNE} & coches & sitios & perros & problemas & niños \\
\texttt{RoBERTa-large-BNE} & coches & sitios & semáforos & peligros & robos \\
\texttt{BETO} & coches & policías & árboles & edificios & niños \\
\texttt{mBERT} & , & niños & barrios & lugares & personas \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} para que le ayudara con los niños."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & hermana & hermano & mujer \\
\texttt{RoBERTa-large-BNE} & madre & padre & hijo & hija & hermana \\
\texttt{BETO} & madre & padre & hermana & hermano & abuela \\
\texttt{mBERT} & padre & madre & hijo & familia & esposa \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} para que le ayudara con la limpieza."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & hermana & mujer & hermano \\
\texttt{RoBERTa-large-BNE} & madre & hijo & padre & mujer & hermana \\
\texttt{BETO} & madre & padre & hermana & hermano & tía \\
\texttt{mBERT} & padre & madre & hijo & amigo & hermano \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} porque se encontraba mal."} \\
\hline
\texttt{RoBERTa-base-BNE} & madre & padre & casa & médico & familia \\
\texttt{RoBERTa-large-BNE} & madre & hijo & puerta & padre & familia \\
\texttt{BETO} & madre & padre & familia & casa & médico \\
\texttt{mBERT} & padre & hijo & hermano & madre & amigo \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Llamó a su \textbf{\{mask\}} porque el coche hacía un ruido raro."} \\
\hline
\texttt{RoBERTa-base-BNE} & padre & madre & mujer & hermano & hermana \\
\texttt{RoBERTa-large-BNE} & madre & padre & hijo & coche & familia \\
\texttt{BETO} & móvil & madre & casa & padre & coche \\
\texttt{mBERT} & coche & familia & padre & casa & madre \\
\bottomrule
\end{tabular}
\end{table}

% las de "llamó a su..." las pensé para evaluar sesgo. la elección de "su" en vez de un artículo es a propósito para que puedan seleccionar un sustantivo de cualquier género. en este sentido, estaría bien poner también el score, para ver si "padre" está muy alejado o no de "madre". como madre, me declaro muy fan de mBERT.


\newpage
\textbf{Lexical selection}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll}
\toprule 
\multicolumn{6}{c}{"Quita las manzanas verdes del cesto y deja solo las \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & rojas & naranjas & verdes & amarillas & nueces \\
\texttt{RoBERTa-large-BNE} & manzanas & de & naranjas & hojas & . \\
\texttt{BETO} & semillas & verdes & manzanas & rojas & malas \\
\texttt{mBERT} & verdes & flores & manos & otras & mismas \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Este es un problema para el cual la solución es \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & sencilla & simple & inmediata & fácil & clara \\
\texttt{RoBERTa-large-BNE} & sencilla & : & fácil & la & simple \\
\texttt{BETO} & simple & sencilla & fácil & desconocida & complicada \\
\texttt{mBERT} & simple & solución & problema & útil & necesaria \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Tenemos un problema para el cual hay que tomar una decisión y hay que \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & solucionarlo & hacerlo & actuar & hablar & esperar \\
\texttt{RoBERTa-large-BNE} & actuar & solucionarlo & hacerlo & resolver & ... \\
\texttt{BETO} & actuar & hacerla & hacerlo & votar & tomar \\
\texttt{mBERT} & decidir & hacerlo & hacer & tomar & pensar \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Felipe \textbf{\{mask\}} que Juan conoce a Marta."} \\
\hline
\texttt{RoBERTa-base-BNE} & dice & cree & asegura & descubre & confiesa \\
\texttt{RoBERTa-large-BNE} & dice & cree & confiesa & afirma & asegura \\
\texttt{BETO} & descubre & dice & sabe & explica & revela \\
\texttt{mBERT} & dice & ordena & indica & de & afirma \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Salió a cazar y mató un \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & león & perro & toro & conejo & gato \\
\texttt{RoBERTa-large-BNE} & león & perro & lobo & hombre & oso \\
\texttt{BETO} & oso & conejo & zorro & león & perro \\
\texttt{mBERT} & hombre & soldado & piloto & caza & home \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Una \textbf{\{mask\}} situada en la región de Alta Normandía."} \\
\hline
\texttt{RoBERTa-base-BNE} & villa & ciudad & localidad & isla & aldea \\
\texttt{RoBERTa-large-BNE} & ciudad & localidad & población & región & villa \\
\texttt{BETO} & francesa & ciudad & localidad & población & comuna \\
\texttt{mBERT} & comuna & localidad & población & parroquia & commune \\
\bottomrule
\toprule 
\multicolumn{6}{c}{"Te voy a contar una \textbf{\{mask\}} sobre mi prima."} \\
\hline
\texttt{RoBERTa-base-BNE} & historia & anécdota & cosa & leyenda & verdad \\
\texttt{RoBERTa-large-BNE} & historia & cosa & anécdota & curiosidad & verdad \\
\texttt{BETO} & historia & cosa & pista & verdad & teoría \\
\texttt{mBERT} & novela & historia & película & pista & cinta \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\textbf{Lexical selection cont'd}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll}
\toprule 
\multicolumn{6}{c}{"Martin se \textbf{\{mask\}} para ir a pescar al río."} \\
\hline
\texttt{RoBERTa-base-BNE} & prepara & ofrece & desnuda & casa & arregla \\
\texttt{RoBERTa-large-BNE} & prepara & preparaba & levanta & ofrece & preparó \\
\texttt{BETO} & prepara & despierta & fue & preparó & preparan \\
\texttt{mBERT} & va & ofrece & encuentra & preparar & queda \\
\bottomrule
\toprule
\multicolumn{6}{c}{"Mi vida no ha sido fácil, pero yo \textbf{\{mask\}} la vida."} \\
\hline
\texttt{RoBERTa-base-BNE} & amo & es & , & soy & quiero \\
\texttt{RoBERTa-large-BNE} & amo & tengo & prefiero & vivo & adoro \\
\texttt{BETO} & amo & soy & vivo & tengo & gano \\
\texttt{mBERT} & es & , & tiene & ama & recuerda \\
\bottomrule
\end{tabular}
\end{table}

\textbf{Polarity agreement}

\begin{table}[!h] \centering \renewcommand{\arraystretch}{1.3} \begin{tabular}{l|lllll} \toprule \multicolumn{6}{c}{"Llegamos muy pronto y no pude hablar con \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & ellos & nadie & vosotros & él & ella \\
\texttt{RoBERTa-large-BNE} & el & ella & ellos & él & nadie \\
\texttt{BETO} & él & ella & nadie & ellos & $[UNK]$ \\
\texttt{mBERT} & ellos & él & ella & nada & ellas \\
\bottomrule
\toprule
\multicolumn{6}{c}{"No lo había visto \textbf{\{mask\}}."} \\
\hline
\texttt{RoBERTa-base-BNE} & nunca & antes & yo & jamás & nadie \\
\texttt{RoBERTa-large-BNE} & nunca & antes & . & ... & yo \\
\texttt{BETO} & antes & nunca & jamás & yo & anteriormente \\
\texttt{mBERT} & él & que & , & ( & por \\
\bottomrule
\end{tabular}
\end{table}

==> tables/sab_polb.tex <==
\begin{table*}[h!]
\centering
\begin{tabularx}{\textwidth}{@{}lrrrrr@{}}
\toprule
Model & \multicolumn{1}{l}{Batch Size} & \multicolumn{1}{l}{Weight decay} & \multicolumn{1}{l}{Learning rate} & \multicolumn{1}{l}{Eval F1}  & \multicolumn{1}{l}{Test F1} \\
\midrule
RoBERTa-b & 16 & 0.01 & 0.00003 & \textbf{0.9167} & \textbf{0.7119} \\
RoBERTa-l & 32 & 0.01 & 0.00003 & 0.9091 & 0.7097 \\
BETO & 32 & 0.1 & 0.00005 & 0.9147 & 0.6667 \\
mBERT & 32 & 0.1 & 0.00005 & 0.8615 & 0.6667 \\
BERTIN & 16 & 0.01 & 0.00005 & 0.8750 & 0.6579 \\
ELECTRA & 32 & 0.01 & 0.00003 & 0.8710 & 0.6102 \\
\bottomrule
\end{tabularx}
\caption{Best configurations for the eval sab-polb dataset with F1 for eval and test.}
\label{tab:evaluation_sab-polb }
\end{table*}


==> tables/tass_detect_polb.tex <==
\begin{table*}[h!]
\centering
\begin{tabularx}{\textwidth}{@{}lrrrrr@{}}
\toprule
Model & \multicolumn{1}{l}{Batch Size} & \multicolumn{1}{l}{Weight decay} & \multicolumn{1}{l}{Learning rate} & \multicolumn{1}{l}{Eval F1}  & \multicolumn{1}{l}{Test F1} \\
\midrule
RoBERTa-b & 16 & 0.01 & 0.00001 & 0.5965 & 0.4776 \\
RoBERTa-l & 32 & 0.1 & 0.00001 & \textbf{0.6275} & \textbf{0.5490} \\
BETO & 16 & 0.01 & 0.00003 & 0.5263 & 0.5135 \\
mBERT & 32 & 0.1 & 0.00001 & 0.3582 & 0.3824 \\
BERTIN & 16 & 0.1 & 0.00003 & 0.4667 & 0.4364 \\
ELECTRA & 16 & 0.1 & 0.00001 & 0.4333 & 0.4667 \\
\bottomrule
\end{tabularx}
\caption{Best configurations for the eval tass-detect-polb dataset with F1 for eval and test.}
\label{tab:evaluation_tass-detect-polb }
\end{table*}


==> tables/tass_sentiment_pol.tex <==
\begin{table*}[h!]
\centering
\begin{tabularx}{\textwidth}{@{}lrrrrr@{}}
\toprule
Model & \multicolumn{1}{l}{Batch Size} & \multicolumn{1}{l}{Weight decay} & \multicolumn{1}{l}{Learning rate} & \multicolumn{1}{l}{Eval Accuracy}  & \multicolumn{1}{l}{Test Accuracy} \\
\midrule
RoBERTa-b & 32 & 0.01 & 0.00003 & 0.7364 & \textbf{0.7413} \\
RoBERTa-l & 16 & 0.01 & 0.00003 & \textbf{0.7442} & 0.7143 \\
BETO & 16 & 0.1 & 0.00005 & 0.7016 & 0.6255 \\
mBERT & 16 & 0.1 & 0.00003 & 0.6473 & 0.6486 \\
BERTIN & 32 & 0.01 & 0.00005 & 0.7364 & 0.7027 \\
ELECTRA & 16 & 0.1 & 0.00003 & 0.7016 & 0.6795 \\
\bottomrule
\end{tabularx}
\caption{Best configurations for the eval tass-sentiment-pol dataset with Accuracy for eval and test.}
\label{tab:evaluation_tass-sentiment-pol }
\end{table*}

